On estimating angular momenta of infalling protostellar cores from observations

We use numerical simulations of molecular cloud formation in the colliding flow scenario to investigate the reliability of observational estimates of the angular momenta of early-state, low-mass protostellar cores. We show that, with suitable corrections for projection factors, molecular line observations of velocity gradients in NH$_3$ can be used to provide reasonable estimates of core angular momenta within a factor of two to three, with a few large underestimates due to unfavorable viewing angles. Our results differ from previous investigations which suggested that observations might overestimate true angular momenta by as much as an order of magnitude; the difference is probably due to the much smoother velocity field on small scales in our simulations, which result from allowing turbulence to decay and gravitational infall to dominate. The results emphasize the importance of understanding the nature of 'turbulent' velocities, with implications for the formation of protostellar disks during core collapse.

==> stuff.tex <==
Unfortunately, depending upon the details of magnetic diffusion, field strengths,
orientation of the field with respect to the angular momentum vector, field geometry,
and possible turbulent motions in protostellar cores,
magnetic fields either a) prevent Keplerian disks of substantial
size from forming due to magnetic braking, b) reduce their extent significantly, c) reduce
sizes mostly at early times, d) have little or no effect, or e) only significantly affect some subset
of the population \citep{allen03,galli06,hennebelle08,
krasnopolsky10,ciardi10,dapp10,dapp12,joos12,li13,santos-lima12,santos-lima13,
seifried12,seifried13,krumholz13,bate14,machida14}.

